Limit theory of sparse random geometric graphs in high dimensions

We study topological and geometric functionals of $l_\infty$-random geometric graphs on the high-dimensional torus in a sparse regime, where the expected number of neighbors decays exponentially in the dimension. More precisely, we establish moment asymptotics, functional central limit theorems and Poisson approximation theorems for certain functionals that are additive under disjoint unions of graphs. For instance, this includes simplex counts and Betti numbers of the Rips complex, as well as general subgraph counts of the random geometric graph. We also present multi-additive extensions that cover the case of persistent Betti numbers of the Rips complex.

==> defs.tex <==
\def\mb{\mathbb}
\def\mc{\mathcal}

\newcommand{\bA}{\mb A}
\newcommand{\bE}{\mb E}
\newcommand{\bF}{\mb F}
\newcommand{\bB}{\mb B}
\newcommand{\bL}{\mb L}
\newcommand{\bM}{\mb M}
\newcommand{\bN}{\mb N}
\newcommand{\bC}{\mb C}
\newcommand{\bP}{\mb P}
\newcommand{\bQ}{\mb Q}
\newcommand{\bR}{\mb R}
\newcommand{\bT}{\mb T}
\newcommand{\bH}{\mb H}
\newcommand{\bD}{\mb D}
\newcommand{\bS}{\mb S}
\newcommand{\bV}{\mb{\hspace{-.07mm}V\hspace{-.2mm}}}

\newcommand{\cA}{\mc A}
\newcommand{\cB}{\mc B}
\newcommand{\cC}{\mc C}
\newcommand{\cD}{\mc D}
\newcommand{\cE}{\mc E}
\newcommand{\cF}{\mc F}
\newcommand{\cG}{\mc G}
\newcommand{\cH}{\mc H}
\newcommand{\cI}{\mc I}
\newcommand{\cL}{\mc L}
\newcommand{\cM}{\mc M}
\newcommand{\cN}{\mc N}
\newcommand{\cV}{\mc V}
\newcommand{\cW}{\mc W}
\newcommand{\cQ}{\mc Q}
\newcommand{\cP}{\mc P}
\newcommand{\cR}{\mc R}
\newcommand{\cS}{\mc S}
\newcommand{\cT}{\mc T}

\newcommand{\E}{\mb E\,}
\newcommand{\R}{\mb R}
\newcommand{\N}{\mb N}
\newcommand{\C}{\mb C}
\newcommand{\Z}{\mb Z}
\newcommand{\s}{\mb S}
\newcommand{\B}{\mb B}
\renewcommand{\P}{\mb P}
\newcommand{\X}{\mb X}
\newcommand{\V}{\mb V}

\newcommand{\dint}{\mathrm{d}}
\def\tff{\uparrow \infty}
\def\tz{\downarrow0}
\def\la{\lambda}
\def\de{\delta}
\def\b{\beta}
\def\bet{\begin{theorem}}
\def\ent{\end{theorem}}
\def\f{\frac}
\def\one{\mathbbmss{1}}
\def\g{\gamma}
\def\bel{\begin{lemma}}
\def\enl{\end{lemma}}
\def\bep{\begin{proof}}
\def\enp{\end{proof}}
\def\Var{\ms{Var}}
\def\ms{\mathsf}
\def\r{\rho}
\def\su{\subseteq}
\def\e{\varepsilon}
\def\bepr{\begin{proposition}}
\def\enpr{\end{proposition}}
\def\ot{[0, 1]}
\def\ff{\infty}
\def\eb{\e_{\ms B}}
\def\kn{\r_d^d}
\def\s{\sigma}
\def\GG{\mc G}
\def\PP{\mc P}
\def\RR{\mc G}
\def\AA{\mc A}
\def\TT{\mc T}
\def\BB{\mc B}
\def\ba{|\,}
\def\Cov{\ms{Cov}}
\def\dist{\ms{dist}}
\def\been{\begin{enumerate}}
\def\enen{\end{enumerate}}
\def\im{\item}
\def\diam{\ms{diam}}
\def\ni{\noindent}
\def\co{\colon}
\def\sm{\setminus}
\def\wt{\widetilde}
\def\De{\Delta}
\def\bnz{\b_{i, d}}
\def\dnz{\De_{i, d}}
\def\rC{r}
\def\d{{\rm d}}
\def\tf{\tfrac}
\def\xx{{\boldsymbol x}}
\def\yy{{\boldsymbol y}}
\def\lrsa{\leftrightsquigarrow}
\def\pa{\partial}
\def\vp{\varphi}
\def\es{\emptyset}
\def\bs{\boldsymbol}
\def\pha{\phantom}
\def\lan{\langle}
\def\t{\tau}
\def\ran{\rangle}
\def\a{\alpha}
\def\dxx{\d\xx}

\definecolor{wiasblue}   {cmyk}{1.0, 0.60, 0, 0}


\newcommand{\blue}[1]{{\textcolor{wiasblue}{{\bf \emph{#1}}}}{}}
\def\bec{\begin{corollary}}
\def\enc{\end{corollary}}


==> task.tex <==

Let $\eta_d$ be a Poisson point process in the unit cube in $\R^d$ of intensity measure $t_d \Lambda_d$, where $\Lambda_d$ denotes the Lebesgue measure.
Let $\delta_d\in (0,\frac{1}{4})$ with $\delta_d\to 0$ as $d\to\infty$.
For $k\in\N_0$, let $F_k$ be the number of $k$-dimensional simplices of the corresponding random simplicial complex $\mathrm{VR}^\infty(\eta_d,\delta_d)$ as defined in Chapter 4 of the thesis \cite{grygierek2019} of Jens Grygierek.

Lemma 4.2.1 of \cite{grygierek2019} provides the bounds
\begin{align} \label{eq0310}
    (1-2\delta)^d \frac{t (t \delta^d)^k (k+1)^d}{(k+1)!}
    \leq \E F_k
    \leq \frac{t (t \delta^d)^k (k+1)^d}{(k+1)!} .
\end{align}

% We deduce that
% \begin{align*}
%     \frac{\E F_k}{\E F_{k-1}}
%     % &\leq \frac{ \frac{t (t \delta^d)^k (k+1)^d}{(k+1)!} }{ (1-2\delta)^d \frac{t (t \delta)^{k-1} k^d}{k!} }\\
%     &\leq (t \delta^d) \left( \frac{k+1}{k} \right)^d \frac{1}{k+1} \left( \frac{1}{1-2\delta} \right)^d.
% \end{align*}
% By iteration this gives
% \begin{align*}
%     \frac{\E F_k}{\E F_1}
%     &\leq (t \delta^d)^{k-1} \left( k+1 \right)^d \frac{2}{(k+1)!} \left( \frac{1}{1-2\delta} \right)^{d(k-1)}.
% \end{align*}
% With the bound $n! \geq \sqrt{2\pi} n^{n} e^{-n}$, %$n! \geq \sqrt{2\pi} n^{n+\frac{1}{2}} e^{-n}$, 
% \begin{align*}
%     \frac{\E F_k}{\E F_1}
%     &\leq (t \delta^d)^{k-1} \left( k+1 \right)^d \sqrt{\frac{2}{\pi}} \left(\frac{e}{k+1}\right)^{k+1} \left( \frac{1}{1-2\delta} \right)^{d(k-1)}.
% \end{align*}

\textbf{(Task 1)} From this we should easily get a statement of the following form.
Let $\bar{\delta}_d = ... \textbf{(?)} $. One has
\begin{align*}
    \E \chi(\delta) 
    = \E \chi(\delta,d,t_d)
    := \sum_{k\in\N_0} (-1)^k \E F_k(\delta)
    & = t_d - \E F_1(\delta) + o(\E F_1(\delta)) ,
    \qquad 0<\delta < \bar{\delta}_d,
\end{align*}
which we can also write as
\begin{align*}
    \E \chi(\delta) - t_d
    & = \frac{t (t \delta)^k (k+1)^d}{(k+1)!} (1+o(1)) ,
    \qquad 0<\delta < \bar{\delta}_d,
\end{align*}
where the small o term is bounded uniformly with respect to $\delta$ by some term going to $0$ as $d\to\infty$.

\bigskip
\textbf{(Task 2)} Jens provides univariate CLT for $F_k$. We would have to extend it to multivariate CLT for $(F_k(\delta_1),\ldots,F_k(\delta_m))$, using the Malliavin-Stein method, at least for $k=1$.

\bigskip
\textbf{(Task 3)} Clarify the following definitions.\\
We set $X_r = X_{r,d,t} = \chi( \text{some function of $r$ and $d$ maybe of the form } r^{1/d} \bar{\delta}_d )$. Here $r$ is a parameter living on a fixed range $(0,T)$.
We normalize the random functions $(X_r)_{0\leq r\leq T}$ in the following way:
\begin{align*}
    \widetilde{X}_r = \frac{X_r - \E X_r}{ F(d)} ,
\end{align*}
where $F(d)$ is a function depending only on $d$ (and maybe also the regime for $d\mapsto t_d$ ?).
The function $F(d)$ should satisfies that it is of the order of the square root of the variance of $X_r$, that is $\sqrt{\V X_r} = \Theta_r(F(d))$.

\bigskip
\textbf{(Task 4)} Show a functional limit theorem.\\
See Theorem 1 and 2 in \cite{krebs} for examples of such theorem.
This might require to get bound looking like $\E (X_r-X_s)^\gamma \overset{!}{\leq} C |r-s|^{1+\epsilon}$ where $\gamma=?$.




==> taskone.tex <==
\section{Task one: The Euler Characteristic is dominated by one term}

Lemma 4.2.1 of \cite{grygierek2019} provides the bounds
\begin{align*}
    (1-2\delta)^d \frac{t (t \delta^d)^k (k+1)^d}{(k+1)!}
    \leq \E F_k
    \leq \frac{t (t \delta^d)^k (k+1)^d}{(k+1)!} , \qquad d\geq 1, \ k\geq 0, \ \delta\in (0,\frac{1}{4}), \ t\in (0,\infty) .
\end{align*}
The bounds are said to hold for any $k\geq 1$. This trivially extends to $k\geq 0$ since $\E F_0 = t$.

We deduce that for any $k\geq 1$
\begin{align} \label{eq:0311}
    \left( t^{\frac{1}{d}} \delta \frac{k+1}{k} (1-2\delta) \right)^d \frac{1}{k+1} 
    &\leq \frac{\E F_k}{\E F_{k-1}}
    \leq \left( t^{\frac{1}{d}} \delta \frac{k+1}{k} \frac{1}{1-2\delta} \right)^d \frac{1}{k+1} .
\end{align}

Recall that $\delta\to 0$ as $d\to\infty$. It implies the following lemma.
\begin{lemma} \label{lem0310}
    Let $k\in\N$ and $\epsilon\in(0,1)$.
    \begin{enumerate}
        \item If $\delta \leq \frac{k}{k+1} t^{-1/d} (1-\epsilon)$ and $d$ is large enough so that $\frac{1-\epsilon}{1-2\delta} \leq 1-\frac{\epsilon}{2}$ then 
        \begin{align*}
            \frac{\E F_k}{\E F_{k-1}}
            & \leq \left( 1 - \frac{\epsilon}{2} \right)^d ,
        \end{align*}
        and, if $d$ is so large that $ \left( 1 - \frac{\epsilon}{2} \right)^{d}
        \leq \left( 1 - \frac{\epsilon}{3} \right)^{d} \left( 1-\left( 1 - \frac{\epsilon}{2} \right)^{d} \right)$ also holds, then
        \begin{align*}
            \sum_{\ell \geq k} \E F_\ell 
            \leq \E F_{k-1} \left( 1 - \frac{\epsilon}{3} \right)^d .
        \end{align*}
        \item If $\delta \geq \frac{k}{k+1} t^{-1/d} (1+\epsilon)$ and $d$ is large enough so that $(1+\epsilon)(1-2\delta)\left(\frac{1}{k+1}\right)^{\frac{1}{d}} \geq 1+\frac{\epsilon}{2} $, then
        \begin{align*}
            \frac{\E F_k}{\E F_{k-1}}
            & \geq \left( 1 + \frac{\epsilon}{2} \right)^d ,
        \end{align*} 
        and, if $d$ is so large that $ \left( 1 - \frac{\epsilon}{2} \right)^{d}
        \leq \left( 1 - \frac{\epsilon}{3} \right)^{d} \left( 1-\left( 1 - \frac{\epsilon}{2} \right)^{d} \right)$ also holds, then
        \begin{align*}
            \sum_{0 \leq \ell \leq k-1} \E F_\ell 
            \leq \E F_{k} \left( 1 - \frac{\epsilon}{3} \right)^d .
        \end{align*}
    \end{enumerate}
\end{lemma}
\begin{proof}
    The first statements of both items follows directly from the bounds \eqref{eq:0311}.
    We get the remaining statements by iterating these bounds and taking the sum of a geometric series.
    Under the conditions of the first item,
    \begin{align*}
        \sum_{\ell \geq k} \E F_\ell
        = \E F_{k-1} \sum_{\ell\geq k} \frac{\E F_\ell}{\E F_{k-1}}
        \leq %\E F_{k-1} \sum_{\ell \geq k} \left( 1 - \frac{\epsilon}{2} \right)^{d (\ell-k)} =
        \E F_{k-1} \sum_{\ell \geq 1} \left( 1 - \frac{\epsilon}{2} \right)^{d \ell}
        = \E F_{k-1} \frac{\left( 1 - \frac{\epsilon}{2} \right)^{d}}{1-\left( 1 - \frac{\epsilon}{2} \right)^{d}}
        \leq \E F_{k-1} \left( 1 - \frac{\epsilon}{3} \right)^{d}. 
    \end{align*}
    Following the same steps, under the conditions of the second item,
    \begin{align*}
        \sum_{0 \leq \ell \leq k-1} \E F_\ell
        \leq \E F_k \sum_{0\leq \ell \leq k-1} \left( 1 - \frac{\epsilon}{2} \right)^{d (k-\ell)}
        \leq \E F_k \sum_{1\leq \ell} \left( 1 - \frac{\epsilon}{2} \right)^{d \ell}
        = \E F_k \frac{\left( 1 - \frac{\epsilon}{2} \right)^{d}}{1-\left( 1 - \frac{\epsilon}{2} \right)^{d}}
        \leq \E F_k \left( 1 + \frac{\epsilon}{3} \right)^{d} .
    \end{align*}
\end{proof}


This essentially means that if $\delta t^{\frac{1}{d}}$ is between $1-\frac{1}{k+1}+\epsilon$ and $1-\frac{1}{k+2}-\epsilon$ then $\E F_k$ dominates all the other $\E F_\ell$. We exploit this to obtain the asymptotic of the Euler characteristic $\chi(\delta) = \sum_{k\in \N_0} (-1)^k F_k $ for any regime $d\mapsto (t_d,\delta_d)$ for which $\delta t^{\frac{1}{d}}$ stays in a compact subset of a connected component of $(0,1) \setminus \{ \frac{2}{3} , \frac{3}{4} , \frac{4}{5}, \ldots \}$.

\begin{lemma} 
    Let $\epsilon > 0 $ and $k \in \N_0$.
    There exists $d_0\in \N$ depending on $k$, $\epsilon$ and the function $d\mapsto (t_d,\delta_d)$ such that the following holds for any $d\geq d_0$.
    \begin{enumerate}
        \item For any $\delta$ with $\delta t^{\frac{1}{d}} \leq 1 - \frac{1}{3} - \epsilon $,
        \begin{align*}
            \left| \chi(\delta) - t + \E F_1 \right| 
            \leq \left( 1 - \frac{\epsilon}{3} \right)^{d} \E F_1 .
            % \leq \frac{t^2 (2\delta)^d}{6} \left( 1 - \frac{\epsilon}{3} \right)^{d} .
        \end{align*}
        \item For any $\delta$ with $ 1 - \frac{1}{k+1} + \epsilon \leq \delta t^{\frac{1}{d}} \leq 1 - \frac{1}{k+2} - \epsilon $,
        \begin{align*}
            \left| \chi(\delta) - (-1)^k \E F_k \right| 
            \leq 2 \left( 1 - \frac{\epsilon}{3} \right)^{d} \E F_k  .
            % \leq \frac{t (t \delta^d)^k (k+1)^d}{(k+1)!} \left( 1 - \frac{\epsilon}{4} \right)^{d} .
        \end{align*}
    \end{enumerate}
\end{lemma}
\begin{proof}
    The first item follows from the first item of Lemma \ref{lem0310} with $k=1$ and the observation that  $\E F_0 = t$.
    For the second item, one observes that
    \begin{align*}
        \left| \chi(\delta) - (-1)^k \E F_k \right| 
        \leq \sum_{0\leq \ell \leq k-1} \E F_\ell + \sum_{k +1 \leq \ell} \E F_\ell 
    \end{align*}
    and bound the two last sums using both items of Lemma \ref{lem0310}.
\end{proof}  
